Technical Report: Benefits of Stabilization versus Rollback in Self-Stabilizing Graph-Based Applications on Eventually Consistent Key-Value Stores

In this paper, we evaluate and compare the performance of two approaches, namely self-stabilization and rollback, to handling consistency violating faults (\cvf) that occur when a self-stabilizing distributed graph-based program is executed on an eventually consistent key-value store. Consistency violating faults are caused by reading wrong values due to weaker level of consistency provided by the key-value store. One way to deal with these faults is to utilize rollback whereas another way is to rely on the property of self-stabilization that is expected to provide recovery from arbitrary states. We evaluate both these approaches in different case studies --planar graph coloring, arbitrary graph coloring, and maximal matching-- as well as for different problem dimensions such as input data characteristics, workload partition, and network latency. We also consider the effect of executing non-stabilizing algorithm with rollback with a similar stabilizing algorithm that does not utilize rollback.

==> experiment-analysis.tex <==
\begin{itemize}
    \item In the later round of stabilization algorithm, only a small number of nodes need to change their states and most other nodes are unchanged (stable nodes).
    By not using mechanism for exclusive access, the clients scan over these stable nodes quickly (since obtaining exclusive access is usually the most time consuming operation for each node). Therefore, the computation is speedup.
    \item Also some \cvf are not harmful. As an example, consider a scenario in graph coloring problem where client $C1$ reads the state/color of node $j$ while client $C2$ is updating the state/color of $j$. This is a \cvf since in sequential consistency, this should not happen when the clients employ exclusive access mechanisms. However, $C2$ does not change the state/color of $j$ since its color is different from all the neighbors. So the state value $j$ read by $C1$ is still consistent.
    For another example, consider a \cvf corresponding to the reading of an inconsistent value of some variables that results in guard $g$ of an action $g \longrightarrow st$ to evaluate to false. The effect of such \cvf is the stuttering of the same state. In stabilization approach, the computation of the program is unaffected by such harmless \cvf while in the detect-rollback approach, since the monitors are not able to classify harmful and harmless \cvf, they triggers unnecessary rollbacks. 
    \item Another factor is the monitors in detect-rollback approach suffers from false positives in detection of \cvf. Therefore, the detect-rollback approach may be not efficient as the stabilization approach.
    \item The detect-rollback approach also is limited to detection of linear and semi-linear predicates.
    \item The benefit of rollback in the random partition depends on specific partition.
    \item Eventual with aggressive stabilization provides the best performance. However, it increases the chance of \cvf and create some \cvf's that are difficult to recover.
    
\end{itemize}


% \textbf{Nature of problems}
% problem where a change has cascading effect like maximal matching

% Problem where a change is local like coloring

% \textbf{Nature of input graph}
% Highly connected graphs such social graph

% Less connected graphs such as planar graph, regular graphs

% \textbf{Impact of graph partition schemes}
% Using Metis partition: requires pre-processing.

% Using normal partition

% The difference between R1W3-ME and R1W1-ME reflects the difference between sequential consistency and eventual consistency. The difference between R1W1-ME and R1W1-noME shows the amount of time needed for coordination between the clients. This amount of time constitute the majority of the computation time. And therefore, the read phase constitute the majority of time of a task.



==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}

A traditional distributed system consists of a set of \textit{nodes} connected to each other by a set of channels. Each node is associated with a set of \textit{variables} and a set of \textit{actions}. These actions read the variables (of that node and possibly other nodes) and update the variables. 
%Continued execution in this manner updates the variables of (possibly) all nodes in a manner as desired by the goals of the system.
{Continued execution in this manner updates the variables of (possibly) all nodes in a computation/procedure that achieves the desired goal of the system.}
%For example, consider a program for distributed maximal matching. In such a program, each node is associated with its matching partner (if any) and other variables to keep track of proposals, timestamps, etc. 
{For example, in a distributed maximal matching program, each node is associated with variables to keep track of its matching partner (if any), proposals, timestamp, etc.}
The program reads these variables to identify which pairs of nodes should be matched with each other. We denote this model as an {the} \textit{active node model}. %Intuitively, the reason is that the nodes appear to be active in updating their own state. 

In \cite{NKD2019ICDCN}, we introduced the notion of a {the} \textit{passive node model} that is targeted towards scenarios where the number of nodes is very large. For example, if we wanted to perform the matching algorithm in a graph of tens or hundreds of thousands of nodes, clearly, having such large active nodes is not feasible. In the passive node model, the variables associated with the nodes are stored in some data store, which in turn could be replicated and/or partitioned. A set of clients operate on this data store to perform the actions as described by the program. 
%For example, in a passive node model for the matching program, the variables associated with the nodes would be stored in a data store. The \textit{clients} will read the relevant variables to determine if matching of one or more node should be changed. The process will continue until a maximal matching is found. 
{For example, in a passive node model for the matching program, the \textit{clients} read the relevant variables from a data store to determine if matching of one or more nodes should be changed. If any variables are changed, the clients write the changes onto the data store.} The process will continue until a maximal matching is found.

In the active %state 
node model, it is assumed that when a node reads the variables of its neighbors, it obtains the latest information about that node. This is reasonable given that there is only one copy of each variable.  The same property could be achieved if we use a single copy (replica) of the data store in the passive node model. %However, maintaining multiple copies is beneficial for many reasons such as fault-tolerance, improved access time and availability of data. When multiple copies are maintained, if we provide sequential consistency, each client will obtain the latest copy of the data. However, sequential consistency requires high overhead whereas a weaker consistency model, e.g., eventual consistency, can substantially increase throughput and reduce latency. However, if we use eventual consistency then a client may obtain stale information about the status of nodes. This is denoted as consistency violation fault (\cvf).
%Preventing \cvf{s}, i.e., preventing access to such stale information essentially requires the use of sequential consistency thereby resulting in an increase of access time and reduction in throughput. 
\duongrephrase{However, most data stores in practice~\cite{DHJKLPSVV07SOSP,LM10SIGOPS,Voldemort,RK18ASE} consist of multiple replicas for many reasons such as fault-tolerance, improved access time and availability of data. When multiple replicas are maintained, clients will obtain fresh data if sequential consistency is enforced for data replication. However, sequential consistency~\cite{??} requires high overhead to resolve discrepancies among replicas, especially in the presence of transient faults (which is a norm in large distributed systems) sequential consistency could result in significant data access delay which makes it inadequate for many applications. A weaker consistency protocol such as eventual consistency~\cite{??} substantially improves the throughput but at the risk of erroneously reading stale data. This kind of error is denoted as consistency violation fault (\cvf). Preventing \cvf{s}, i.e., preventing access to stale data, essentially requires the enforcement of sequential consistency and thereby retards the performance.}

%Since preventing the use of stale information is not desirable, there are two ways of dealing with such stale information.
One approach to 
%deal with this challenge 
handle \cvf is to detect the use of such stale 
%information
data. 
%This can be achieved by using algorithms such as those in \cite{CG98DC}. To achieve this, we need to run a monitor concurrently with the program. When the monitor detects a violation, we can restore the program to a previous state and continue the execution thereafter. 
\duongrephrase{A monitor runs concurrently with the program and implements predicate detection algorithms such as those in~\cite{CG98DC} to detect instances of \cvf. When a violation (\cvf) is detected, the program is restored to a previous state that is correct and continues its execution thereafter. In~\cite{NCKD2019JBCS}, the authors demonstrated that for graph-based applications such detect-rollback approach is feasible since detection and recovery could be done efficiently.}
%%% Some of the text below is moved to Section \ref{sec:sys-model-architecture}
%In \cite{NCKD2018LADC}, the authors found that the detection of the violation is often very quick. Specifically, it is possible to restart a few actions taken by clients involved in conflicting access to data rather than requiring all clients to rollback in a coordinated fashion. (We refer the reader to Section \ref{sec:detect-rollback} for details.)
%
An alternate approach is to use stabilization~\cite{EDW426}. A stabilizing program is guaranteed to recover from an arbitrary state to a legitimate state. Thus, if a client ends up \duongnote{executing a \cvf} (updating the information of some node based on stale information), 
%we can treat it 
\duongrephrase{the \cvf can be treated} 
as if a fault caused the state of that node to be perturbed. A stabilizing program is designed to recover from such a fault as long as such faults do not occur frequently. (We refer the reader to Sections~\ref{sec:cvf} and \ref{sec:detect-rollback} for more details about stabilization and rollback.)
\duongtodo{I have moved some text that discusses rollback and stabilization to Section~\ref{sec:sys-model-architecture}}.
%%% The text below is moved to Section\ref{sec:sys-model-architecture}
%Specifically, a stabilizing program is guaranteed to recover after the faults stop (or if faults do not occur for a long enough time). If the \cvf{s} occur frequently then the program may not be able to recover from them. At the same time, given the nature of \cvf{s}, expecting them to never occur during recovery is not reasonable. 
%Thus, we need to evaluate how \cvf{s} perturb the recovery to determine the overall effect \duongtodo{We do not have this evaluation in this paper?}. 
%In \cite{NKD2019ICDCN}, it is shown that the perturbation caused by \cvf{s} is not as severe in the sense that tolerating \cvf{s} and using eventual consistency is better than eliminating \cvf{s} with sequential consistency. 

\textbf{Summary of the main results.} 
In this paper, we %focus on 
investigate
%the tradeoff between these two approaches. %%% I think the paper is not about the tradeoff since rollback does not perform as well asstabilization in this paper experiments
the benefits of the two approaches in handling \cvf{s}.
Clearly, if the underlying program is not stabilizing then we must 
%utilize the rollback-recovery based approach. 
rely on the detect-rollback approach.
Hence, we %consider 
focus on stabilizing programs where both approaches are %feasible. 
applicable.
Specifically, we %focus on 
consider three stabilizing \duongtodo{is the term stabilizing program and self-stabilizing program equivalent?} graph-based applications: planar graph coloring, arbitrary graph coloring, and maximal matching.
We run experiments on LinkedIn's Voldemort key-value store on our local network and Amazon Web Service (AWS) network.
The source code and experimental results are available at \cite{Nguyen20ZenodoICDCS}. 
From the experimental results, we observe the followings:
\duongrephrase{
\begin{itemize}
    \item Stabilization approach provides higher benefits than the rollback approach in the case studies used in this paper. Using sequential consistency as the base-line for comparison, stabilization improves the convergence time of the applications by 25~\% to 35~\%, whereas the rollback approach improves the convergence time by 30~\% in the best case and potentially causes performance to suffer.
    \item 
    %Enforcing/Realizing the atomicity requirement (clients are not allowed to update the state of neighboring nodes simultaneously-- cf. Section~\ref{sec:distprogram}) constitutes a significant proportion of the client computation.
    We observe a sizeable proportion of the computation time is spent on coordination operations by the clients to ensure the action atomicity requirement is satisfied (clients do not update the states of neighboring nodes simultaneously-- cf. Section~\ref{sec:distprogram}). In stabilization, we take a further step that removes coordination operations from the clients and treats violations of the action atomicity requirement as additional \cvf{s}. This aggressive stabilization approach 
    %trades the recovery cost of the additional \cvf{s} for the elimination of the coordination overhead.
    eliminates the coordination overhead at the cost of more recovery time for the extra \cvf{s}.
    Experimental results show that the cost of extra \cvf{s} is outweighed by the benefits of no coordination overhead. Specifically, the convergence time of the applications speeds up by 2 to 15 times with aggressive stabilization.
    \item {\color{red} We further analyze the \cvf{s} caused by the removal of client coordination and find that many of them resolve favorably by themselves, thus reducing the stabilization cost. By contrast, the rollback approach }

\end{itemize}
}

\begin{itemize}
    % \item {\color{red}{Add discussion on selection representative for Rollback and when Rollback may be beneficial.}}
    \item For the case study applications used in this paper, we observe that the stabilization approach is better than the detect-rollback approach, especially when we treat violations of atomicity requirement (e.g. violation of mutual exclusion where the same data item is concurrently accessed by two clients) as \cvf{s}. Specifically, the stabilization approach improves the convergence time (compared to running on sequential consistency) by \SI{25}{\percent} to \SI{35}{\percent}. With aggressive stabilization approach, convergence time is sped up by 2 to 15 times. By contrast, the detect-rollback approach improves convergence time by 30\% in the best case, and potentially causes performance to suffer when compared with sequential consistency.

    The reason for this difference is that securing the atomicity of actions contribute a significant amount of time in the computation. By eliminating this requirement, the computation time is boosted. On the other hand, without the atomicity requirement, the clients can read inconsistent data and produce incorrect results. In the self-stabilization approach, these incorrect results are treated as \cvf{s} and handled automatically. 
    %which result in additional recovery time. However, this overhead is outweighed by the computation time reduction due to the elimination of the atomicity requirement. 
    By contrast, since the rollback approach requires these mechanisms to detect possible violations, this approach is not able to utilize such benefit of eliminating atomicity requirement.
    %The key reason for this difference is that obtaining locks constitutes the majority ({\color{red}{an overwhelming majority, about 90 \si{\percent}}}) of the application computation time. By eliminating the mutual exclusion mechanism, the computation time is significantly improved. On the other hand, without the mutual exclusion mechanism, the chance of clients reading inconsistent data is increased. In the self-stabilization approach, these inconsistencies can be treated as \cvf. They increase the recovery time. However, this overhead is outweighed by the computation time reduction due to the elimination of the mutual exclusion requirement. By contrast, since the rollback recovery approach requires mutual exclusion mechanisms to detect possible violations and trigger the rollback, this approach is not able to utilize the benefit of eliminating mutual exclusions.
    \item We analyze different factors that affect the performance of both approaches such as input graph, type of applications, partitioning scheme, and network latency. 
    We find that on graphs with complex connectivity between nodes such as social graphs, the overhead of guaranteeing the atomicity requirement is high, and the stabilization approach performs well since it eliminates that overhead. By contrast, the detect-rollback approach suffers from higher chance of violations as well as a significant amount of work wasted during rollbacks. In regular graphs, the overhead of mutual exclusion is reduced and the detect-rollback provides some benefit. We also find that the benefits of both approaches are improved if we employ a partitioning scheme that distributes the partitions among the clients evenly and/or preserves the locality of the graph. When the network latency increases, we observe the benefits of stabilization improve while the benefits of rollback may increase or decrease, depending on the application.
    %Impact of application type and input graphs. When the input is a regular graph where each node has roughly the same degree, we observe that the benefit of rollback approach is from \SI{16}{\percent} to \SI{29}{\percent}. These are almost comparable to the benefit of the self-stabilization approach with locks enabled (\SI{26}{\percent} to \SI{34}{\percent}). However, when the input is a social graph where the connectivity of nodes follows the power-law distribution, the time for obtaining locks \todo{} relevant to high degree nodes is very large. Consequently, if the violation occurs and the program is rolled back, the amount of work wasted is large. Thus, the performance of the rollback approach is only comparable or even worse than using sequential consistency. On the other hand, the approach of self-stabilization without mutual exclusion achieves the highest speedup because it avoids the overhead of locking.
    \item Although being more beneficial, the stabilization approach could suffer from some rare \cvf{s} that prevent the application to converge. In such cases, we propose some heuristics, such as randomization and tracking the update timestamps of active neighbor nodes, to improve the performance of stabilization.
    %Although the approach of self-stabilization with mutual exclusion disabled provides the best performance, in some application such as graph coloring on an arbitrary graph, the program may not stabilize. In this case, we propose to use some randomization to provide probabilistic convergence.
    %\item In the passive node model, the nodes are processed by the clients in rounds, i.e. each client processes one node at a time in some order. In the later rounds, the number of enabled nodes, i.e. nodes that have to change its state, is only a small fraction of the total number of nodes. Hence, a large amount of time spent on disabled nodes to obtain locks and read neighbors state is practically useless. In this case, we can augment the algorithm with additional variables tracking the state changes of nodes and their neighbors so that clients only process nodes whose neighbor's states have change recently. The augmented variables have their own overhead but can avoid some wasted amount of work. Our experiment results show that using augmented variables is beneficial for the self-stabilization approach with mutual exclusion disabled. 
    %\item Benefit of additional information about the structure of input: list of high degree nodes, existing efficient partitioning schemes. These can reduce the number of locks, and thus reduce computation time.
\end{itemize}

\textbf{Contributions of the paper.} To the best of our knowledge, our paper is the first to compare the benefits of self-stabilization and rollback in handling data anomalies when running graph-based applications on eventually consistent data stores. We find that when the self-stabilization option is available, it usually provides a better benefit than the detect-rollback recovery approach. Moreover, if we aggressively disable mechanisms for atomicity requirements of actions and treated the violations as other \cvf faults, the stabilization approach outperforms the detect-rollback approach. However, in some applications, self-stabilization algorithms do not exist. In such circumstances, the rollback approach may be the choice. We also analyze different factors that affect the performance of both approaches so that a system designer should consider to have a better design decision.

\textbf{Organization of the paper.} In Section \ref{sec:sys-model-architecture}, we present the system models/architecture, the definition of \cvf, and briefly recall the stabilization and detect-rollback approach. In Section \ref{sec:expriment}, we present and analyze the experimental results. Finally, we conclude the paper in Section \ref{sec:concl}.



==> intro-older.tex <==
A traditional distributed system consists of a set of \textit{nodes} connected to each other by a set of channels. Each node is associated with a set of \textit{variables} and a set of \textit{actions}. These actions read the variables (of that node and possibly other nodes) and update the variables. Continued execution in this manner updates the variables of (possibly) all nodes in a manner as desired by the goals of the system.
For example, consider a program for distributed maximal matching. In such a program, each node is associated with its matching partner (if any) and other variables to keep track of proposals, timestamps, etc. The program reads these variables to identify which pairs of nodes should be matched with each other. We denote this model as an \textit{active node model}. %Intuitively, the reason is that the nodes appear to be active in updating their own state. 

In \cite{NKD2019ICDCN}, we introduced the notion of a \textit{passive node model} that is targeted towards scenarios where the number of nodes is very large. For example, if we wanted to perform the matching algorithm in a graph of tens or hundreds of thousands of nodes, clearly, having such large active nodes is not feasible. In the passive node model, the variables associated with the nodes are stored in some data store, which in turn could be replicated and/or partitioned. A set of clients operate on this data store to perform the actions as described by the program. For example, in a passive node model for the matching program, the variables associated with the nodes would be stored in a data store. The \textit{clients} will read the relevant variables to determine if matching of one or more node should be changed. The process will continue until a maximal matching is found. 

In the active state model, it is assumed that when a node reads the variables of its neighbors, it obtains the latest information about that node. This is reasonable given that there is only one copy of each variable.  The same property could be achieved if we use a single copy of the data store in the passive node model. However, maintaining multiple copies is beneficial for many reasons such as fault-tolerance, improved access time and availability of data. When multiple copies are maintained, if we provide sequential consistency, each client will obtain the latest copy of the data. However, sequential consistency requires high overhead whereas a weaker consistency model, e.g., eventual consistency, can substantially increase throughput and reduce latency. However, if we use eventual consistency then a client may obtain stale information about the status of nodes. This is denoted as consistency violation fault (\cvf).
Preventing \cvf{s}, i.e., preventing access to such stale information essentially requires the use of sequential consistency thereby resulting in an increase of access time and reduction in throughput. 

%Since preventing the use of stale information is not desirable, there are two ways of dealing with such stale information.
One approach to deal with this challenge is to detect the use of such stale information. This can be achieved by using algorithms such as those in \cite{CG98DC}. To achieve this, we need to run a monitor concurrently with the program. When the monitor detects a violation, we can restore the program to a previous state and continue the execution thereafter. In \cite{NCKD2018LADC}, the authors found that the detection of the violation is often very quick. Specifically, it is possible to restart a few actions taken by clients involved in conflicting access to data rather than requiring all clients to rollback in a coordinated fashion. (We refer the reader to Section \ref{sec:detect-rollback} for details.)
An alternate approach is to use stabilization \cite{EDW426}. A stabilizing program is guaranteed to recover from an arbitrary state to a legitimate state. Thus, if a client ends up updating the information of some node based on stale information, we can treat it as if a fault caused the state of that node to be perturbed. A stabilizing program is designed to recover from such a fault as long as such faults do not occur frequently. Specifically, a stabilizing program is guaranteed to recover after the faults stop (or if faults do not occur for a long enough time). If the \cvf{s} occur frequently then the program may not be able to recover from them. At the same time, given the nature of \cvf{s}, expecting them to never occur during recovery is not reasonable. Thus, we need to evaluate how \cvf{s} perturb the recovery to determine the overall effect \duongtodo{We do not have this evaluation in this paper?}. 
%In \cite{NKD2019ICDCN}, it is shown that the perturbation caused by \cvf{s} is not as severe in the sense that tolerating \cvf{s} and using eventual consistency is better than eliminating \cvf{s} with sequential consistency. 

\textbf{Summary of the main results.} 
In this paper, we focus on the tradeoff between these two approaches. Clearly, if the underlying program is not stabilizing then we must utilize the rollback-recovery based approach. Hence, we consider stabilizing programs where both approaches are feasible. Specifically, we focus on three self-stabilizing graph-based applications: namely planar graph coloring, arbitrary graph coloring, and maximal matching.
We run experiments on LinkedIn's Voldemort key-value store on our local network and Amazon Web Service (AWS) network.
The source code and experimental results are available at \cite{Nguyen20ZenodoICDCS}. 
From the experimental results, we observe the followings:
\begin{itemize}
    % \item {\color{red}{Add discussion on selection representative for Rollback and when Rollback may be beneficial.}}
    \item For the case study applications used in this paper, we observe that the stabilization approach is better than the detect-rollback approach, especially when we treat violations of atomicity requirement (e.g. violation of mutual exclusion where the same data item is concurrently accessed by two clients) as \cvf{s}. Specifically, the stabilization approach improves the convergence time (compared to running on sequential consistency) by \SI{25}{\percent} to \SI{35}{\percent}. With aggressive stabilization approach, convergence time is sped up by 2 to 15 times. By contrast, the detect-rollback approach improves convergence time by 30\% in the best case, and potentially causes performance to suffer when compared with sequential consistency.

    The reason for this difference is that securing the atomicity of actions contribute a significant amount of time in the computation. By eliminating this requirement, the computation time is boosted. On the other hand, without the atomicity requirement, the clients can read inconsistent data and produce incorrect results. In the self-stabilization approach, these incorrect results are treated as \cvf{s} and handled automatically. 
    %which result in additional recovery time. However, this overhead is outweighed by the computation time reduction due to the elimination of the atomicity requirement. 
    By contrast, since the rollback approach requires these mechanisms to detect possible violations, this approach is not able to utilize such benefit of eliminating atomicity requirement.
    %The key reason for this difference is that obtaining locks constitutes the majority ({\color{red}{an overwhelming majority, about 90 \si{\percent}}}) of the application computation time. By eliminating the mutual exclusion mechanism, the computation time is significantly improved. On the other hand, without the mutual exclusion mechanism, the chance of clients reading inconsistent data is increased. In the self-stabilization approach, these inconsistencies can be treated as \cvf. They increase the recovery time. However, this overhead is outweighed by the computation time reduction due to the elimination of the mutual exclusion requirement. By contrast, since the rollback recovery approach requires mutual exclusion mechanisms to detect possible violations and trigger the rollback, this approach is not able to utilize the benefit of eliminating mutual exclusions.
    \item We analyze different factors that affect the performance of both approaches such as input graph, type of applications, partitioning scheme, and network latency. 
    We find that on graphs with complex connectivity between nodes such as social graphs, the overhead of guaranteeing the atomicity requirement is high, and the stabilization approach performs well since it eliminates that overhead. By contrast, the detect-rollback approach suffers from higher chance of violations as well as a significant amount of work wasted during rollbacks. In regular graphs, the overhead of mutual exclusion is reduced and the detect-rollback provides some benefit. We also find that the benefits of both approaches are improved if we employ a partitioning scheme that distributes the partitions among the clients evenly and/or preserves the locality of the graph. When the network latency increases, we observe the benefits of stabilization improve while the benefits of rollback may increase or decrease, depending on the application.
    %Impact of application type and input graphs. When the input is a regular graph where each node has roughly the same degree, we observe that the benefit of rollback approach is from \SI{16}{\percent} to \SI{29}{\percent}. These are almost comparable to the benefit of the self-stabilization approach with locks enabled (\SI{26}{\percent} to \SI{34}{\percent}). However, when the input is a social graph where the connectivity of nodes follows the power-law distribution, the time for obtaining locks \todo{} relevant to high degree nodes is very large. Consequently, if the violation occurs and the program is rolled back, the amount of work wasted is large. Thus, the performance of the rollback approach is only comparable or even worse than using sequential consistency. On the other hand, the approach of self-stabilization without mutual exclusion achieves the highest speedup because it avoids the overhead of locking.
    \item Although being more beneficial, the stabilization approach could suffer from some rare \cvf{s} that prevent the application to converge. In such cases, we propose some heuristics, such as randomization and tracking the update timestamps of active neighbor nodes, to improve the performance of stabilization.
    %Although the approach of self-stabilization with mutual exclusion disabled provides the best performance, in some application such as graph coloring on an arbitrary graph, the program may not stabilize. In this case, we propose to use some randomization to provide probabilistic convergence.
    %\item In the passive node model, the nodes are processed by the clients in rounds, i.e. each client processes one node at a time in some order. In the later rounds, the number of enabled nodes, i.e. nodes that have to change its state, is only a small fraction of the total number of nodes. Hence, a large amount of time spent on disabled nodes to obtain locks and read neighbors state is practically useless. In this case, we can augment the algorithm with additional variables tracking the state changes of nodes and their neighbors so that clients only process nodes whose neighbor's states have change recently. The augmented variables have their own overhead but can avoid some wasted amount of work. Our experiment results show that using augmented variables is beneficial for the self-stabilization approach with mutual exclusion disabled. 
    %\item Benefit of additional information about the structure of input: list of high degree nodes, existing efficient partitioning schemes. These can reduce the number of locks, and thus reduce computation time.
\end{itemize}

\textbf{Contributions of the paper.} To the best of our knowledge, our paper is the first to compare the benefits of self-stabilization and rollback in handling data anomalies when running graph-based applications on eventually consistent data stores. We find that when the self-stabilization option is available, it usually provides a better benefit than the detect-rollback recovery approach. Moreover, if we aggressively disable mechanisms for atomicity requirements of actions and treated the violations as other \cvf faults, the stabilization approach outperforms the detect-rollback approach. However, in some applications, self-stabilization algorithms do not exist. In such circumstances, the rollback approach may be the choice. We also analyze different factors that affect the performance of both approaches so that a system designer should consider to have a better design decision.

\textbf{Organization of the paper.} In Section \ref{sec:sys-model-architecture}, we present the system models/architecture, the definition of \cvf, and briefly recall the stabilization and detect-rollback approach. In Section \ref{sec:expriment}, we present and analyze the experimental results. Finally, we conclude the paper in Section \ref{sec:concl}.



==> tocheck.tex <==
\color{red}

TO BE CHECKED AFTER FINISH:

%Use stabilization approach instead of self-stabilization. Use self-stabilizing application.

Need to clarify why \cvf corresponds to the case when the possession time intervals of two clients for the same lock overlapped.

Should say \cvf correspond to the case when the atomicity requirement is violated.

Also atomicity is just one case (remark 2). Remark 1 is reading inconsistent values. We need to clarify this with examples in appendix.

Distinguish between linearizability and sequential consistency.

Differing sequential consistency and linearizability:

(1) what is sequential consistency? Is Lamport's definition of sequential consistency applicable for key-value store? i.e. processor sequential consistency the same as data sequential consistency?

(2) Is data sequential consistency and mutual exclusion (two clients not updating two neighboring nodes simultaneously) sufficient to provide atomicity?  Is this combination equivalent to linearizability?

(3) Also what is the definition of atomicity (by Dolev)? Does atomicity has several variants (i.e. read/write, composite atomicity, etc.)? If it does, then which one should we use, and why?

(4) Is R1W3 in Voldemort provides sequential consistency? If R1W3 client receives 2 different responses from 2 server, what will happen? It returns multi-version value, right? If so, how my current application such as coloring handle multi-version value?



Benchmark: since the algorithm is self-stabilization, we do not have benchmark programs. But we can use benchmark input graphs. May be convert traffic network into planar graphs.

%Is stabilizing and self-stabilizing the same term? Yes

%Replace applications by problems or programs.

%Replace social network graph by social graph.

%Replace eventual with stablization by stablization. Eventual with aggressive stabilization by aggressive stabilization?

\color{black}
